SmmPack: Obfuscation for SMM Modules with TPM Sealed Key

System Management Mode (SMM) is the highest-privileged operating mode of x86 and x86-64 processors. Through SMM exploitation, attackers can tamper with the Unified Extensible Firmware Interface (UEFI) firmware, disabling the security mechanisms implemented by the operating system and hypervisor. Vulnerabilities enabling SMM code execution are often reported as Common Vulnerabilities and Exposures (CVEs); however, no security mechanisms currently exist to prevent attackers from analyzing those vulnerabilities. To increase the cost of vulnerability analysis of SMM modules, we introduced SmmPack. The core concept of SmmPack involves encrypting an SMM module with the key securely stored in a Trusted Platform Module (TPM). We assessed the effectiveness of SmmPack in preventing attackers from obtaining and analyzing SMM modules using various acquisition methods. Our results show that SmmPack significantly increases the cost by narrowing down the means of module acquisition. Furthermore, we demonstrated that SmmPack operates without compromising the performance of the original SMM modules. We also clarified the management and adoption methods of SmmPack, as well as the procedure for applying BIOS updates, and demonstrated that the implementation of SmmPack is realistic.

==> 04_requirements.tex <==
% \section{Requirements} \label{requirements}
\section{Requirements for SmmPack} \label{sec:requirements}
SmmPack is an SMM module obfuscation technique designed to prevent attackers from identifying vulnerabilities, such as those listed in the CVE database. The technical requirements that SmmPack must meet are summarized as follows:

~\\
\noindent{\bf Req 1 (confidentiality)}: Attackers should be prevented from analyzing the code of SMM modules.

\noindent{\bf Req 2 (functionality)}: Packed SMM modules must function correctly. 

\noindent{\bf Req 3 (minimal overhead)}: A realistic boot time and BIOS size must be preserved.\\


\subsection{Req 1: Confidentiality}
To satisfy the first requirement, it is necessary to prevent as many methods as possible for acquiring SMM modules used by attackers from class 1 to class 3, as defined in the previous threat model.
% When evaluating using this threat model, the following assumptions are made.
% \begin{itemize}
%     \item TPM module is tamper resistant.
%     \item Attacks on cryptographic algorithms itself are considered out-of-scope.
%     \item The integrity of SEC and PEI phase (IBB) is hardware protected by Intel Boot Guard or AMD PSB.
% \end{itemize}
When evaluating using this threat model, the following assumptions are made: (1) the TPM module is tamper-resistant, (2) attacks on cryptographic algorithms themselves are considered out-of-scope, and (3) the integrity of the SEC and PEI phases (IBB) is hardware-protected by the Intel Boot Guard or AMD PSB.

We consider attacks targeting the vulnerabilities of TPM and attacks on the cryptographic algorithms themselves to be out-of-scope. Additionally, we assume that hardware-based security mechanisms such as Intel Boot Guard or AMD PSB, which prevent the manipulation of TPM PCR values during the initial boot phases, such as SEC or PEI, are enabled. These are described further in Section \ref{sec:discussion}.



\subsection{Req 2: Functionality}
To satisfy the second requirement, it is necessary to define the conditions that indicate whether the SMM modules function properly.
% The conditions for determining that a SMM module is functioning correctly are as follows:
% \begin{itemize}
%     \item The module can execute from the entry point to the end without stopping.
%     \item The BIOS, including the packed modules, properly boots without stopping.
%     \item The protocol installed by the packed module can be located, and when called, it executes its processing content correctly.
%     \item The SMI handler of the packed module can execute its processing content correctly in response to the SMI.
% \end{itemize}
The conditions for determining whether an SMM module is functioning correctly are as follows: (1) the module can execute from the entry point to the end without stopping, (2) The BIOS, including the packed modules, properly boots without stopping, (3) The protocol installed by the packed module can be located, and when called, it executes its processing content correctly, and (4) The SMI handler of the packed module can execute its processing content correctly in response to the SMI.



\subsection{Req 3: Minimal Overhead}
To fulfill the third requirement, it is necessary to establish criteria for what constitutes realistic boot time and size. In the experimental environment described in Section \ref{sec:implementation}, it took approximately 13 s from pressing the Power button until the Windows login screen was displayed. In this study, if the boot-time overhead of SmmPack is less than 10\% within 13 s, it is considered acceptable. Regarding size overhead, because the number of SMM modules varies for each BIOS, the size overhead of several SMM modules is deemed acceptable. SMM modules have different sizes, but even the largest modules used in this experiment were less than 100.000 bytes. Therefore, an overhead of less than 100.000 bytes can be considered negligible, because it is approximately equivalent to adding a single larger SMM module.

==> 07_func.tex <==
\section{Functionality Assessment (Req 2)}
This section demonstrates that SmmPack satisfies the second requirement defined in Section \ref{sec:requirements}. First, we will outline the experimental methodology for confirming the functionality of the packed SMM module. Subsequently, experimental results are presented.

\subsection{Experimental method}
The experiment utilized the UP Squared Pro board and its BIOS, as shown in Figure \ref{tab:env}.
We implemented an SMM module (TestSmm) that outputs debug messages and installs its own protocol and SMI handler. If TestSmm is packed using SmmPack and the debug messages are displayed, followed by the successful booting of the operating system, it confirms the proper operation of the packed TestSmm. Similarly, by verifying that debug messages from the protocol and SMI handler are output when these are utilized by external modules, it can be confirmed that the protocol and SMI handler installed by the packed TestSmm are functioning correctly.

% The SMM modules used for testing (TestSmm) were built using EDK2, packed by SmmPack's packer, and inserted into the BIOS using UEFITools \cite{uefitool}. To evaluate with a platform-independent general-purpose SMM module, we utilized a module built using EDK2 instead of those within the BIOS. In addition, we created another SMM module that locates and uses the protocol registered by the packed SMM module and inserts it into the BIOS.

% TestSmm outputs debug messages, installs its own protocol, and registers the SMI handler. If the debug message of the packed TestSmm is printed, it confirms that it is operating properly. After the debug message is printed, if the OS or UEFI shell etc. is started, we can confirm that the BIOS, including the packed SMM modules, runs normally without stopping.
% To verify whether the protocol registered by TestSmm operates correctly, it can be determined by calling a function of this protocol from a different SMM module and observing whether the debug output of that function is displayed. 
% Regarding the SMI handler, if the registered SMI handler of the packed TestSmm module is invoked from other UEFI modules and if debug output from the SMI handler is displayed, it confirms that the SMI handler is functioning correctly.
% Regarding the SMI handler, if the registered SMI handler of the TestSmm module is called by other UEFI modules and the handler's debug output is displayed, this verifies the proper functioning of the SMI handler.


\subsection{Experimental results}
As a result, it was confirmed that all debug messages were output, and TestSmm operated correctly even when packed. Based on these results, we conclude that the second requirement in Section \ref{sec:requirements} is satisfied.
%Consequently, the debug output from TestSmm was displayed, and the BIOS containing these modules was successfully booted to the OS or UEFI Shell. Debug messages were also displayed when the protocols installed using TestSmm were located and used from another SMM module. In addition, debug messages from SMI handlers were displayed in response to SMIs. Based on these results, we conclude that the second requirement in Section \ref{sec:requirements} is satisfied.
